Simulation Algorithms with Exponential Integration for Time-Domain Analysis of Large-Scale Power Delivery Networks

We design an algorithmic framework using matrix exponentials for time-domain simulation of power delivery network (PDN). Our framework can reuse factorized matrices to simulate the large-scale linear PDN system with variable stepsizes. In contrast, current conventional PDN simulation solvers have to use fixed step-size approach in order to reuse factorized matrices generated by the expensive matrix decomposition. Based on the proposed exponential integration framework, we design a PDN solver R-MATEX with the flexible time-stepping capability. The key operation of matrix exponential and vector product (MEVP) is computed by the rational Krylov subspace method. To further improve the runtime, we also propose a distributed computing framework DR-MATEX. DR-MATEX reduces Krylov subspace generations caused by frequent breakpoints from a large number of current sources during simulation. By virtue of the superposition property of linear system and scaling invariance property of Krylov subspace, DR-MATEX can divide the whole simulation task into subtasks based on the alignments of breakpoints among those sources. The subtasks are processed in parallel at different computing nodes without any communication during the computation of transient simulation. The final result is obtained by summing up the partial results among all the computing nodes after they finish the assigned subtasks. Therefore, our computation model belongs to the category known as Embarrassingly Parallel model. Experimental results show R-MATEX and DR-MATEX can achieve up to around 14.4X and 98.0X runtime speedups over traditional trapezoidal integration based solver with fixed timestep approach.

==> adaptive_step_control.tex <==

The new proposed MEXP for the power grid simulation can significantly benefit from the adaptive step size control because 
the rational Krylov subspace still preserves the capability of adaptivity, which has been demonstrated the effectiveness 
in linear circuits~\cite{Weng12_TCAD}. And, with the relaxation of the stiffness constraint, MEXP can now utilize even larger 
step size, e.g., 1\emph{ns}, to perform transient analysis. Such large step size is particularly useful for the power grid 
simulation where the voltage noise usually includes the low frequency behavior of both package and board levels. 

The idea of our adaptive step scheme is to step forward as much as possible so that MEXP can finish the simulation 
quickly. With the insight from Eqn. (\ref{eq:scale}), MEXP is able to adjust $\alpha$ to calculate result of arbitrary 
step size with only performing one Arnoldi process. However, because MEXP has to guarantee slopes of input sources must 
be constant within the step size, the maximum allowed step size is limited. Therefore, MEXP will first compute the rational 
Krylov subspace using $\mbf{x}(t)$, and then results within the maximum allowed step size, which is determined by input 
sources, can be calculated through the step size scaling. 

Algorithm~\ref{algo:adaptive_step} shows MEXP with adaptive step control scheme. In order to comply with the required 
accuracy during the simulation, the allowed error $err_k$ at certain time instant $t_k$ is defined as 
\begin{eqnarray}
    err_k \le \frac{E_{Tol}}{T}\times h_k, \nonumber
\end{eqnarray}
where $E_{Tol}$ is the error tolerance in the whole simulation process, $T$ is the simulation time span, $h_k$ is the 
step size at time $t_k$, and $err_k$ is the posterior error of MEXP from Eqn. (\ref{eq:post_err_est}). Hence, when 
we construct the rational Krylov subspace at the current time, we will increase $m$ until the $err_k$ satisfies the 
error tolerance. 

\begin{algorithm} 
    \label{algo:adaptive_step}
    \caption{MEXP with Adaptive Step Control}
    \KwIn{$\mbf{C}$, $\mbf{G}$, $\mbf{B}$, $\mbf{u}(t)$, $\tau$, error tolerance $E_{Tol}$ and simulation time $T$}
    \KwOut{$\mbf{x}(t)$}
    {
        $t = 0$; 
	$\mbf{x}(0)$ = DC\_analysis\;
        %Choose $\tau$ for rational Krylov subspace method\;
        $[\mbf{L}_{sub},\mbf{U}_{sub}] = $LU($\mbf{C} +\gamma \mbf{G}$)\;
        \While{$t \leq T$}
        {	
	    %Update $v_{k+1}$ with $\mbf{L}, \mbf{U}, \mbf{W}$ by (\ref{eq:blu_f})\;
	    %and update $\mathbf{L},\mathbf{U}$ by (\ref{eq:blu})\;
	    Compute maximum allowed step size $h$ from $\mbf{u}(t)$\;
	    Construct $\mbf{H_m}$, $\mbf{V_m}$ by Arnoldi process until $err_k \le \frac{E_{Tol}}{T}h$\;

	    $\alpha = \frac{h}{\gamma}$ \;
	    Compute $\mbf{x}(t+h)$ by (\ref{eq:scale})\;

	    $t = t+h$; 
	}
    }
\end{algorithm}
The complexity of MEXP with adaptive step size is mainly determined by the total number of required backward/forward
substitutions during the simulation process. This is because the dimension of $\mbf{H_m}$ is small, e.g., around 
$5 \sim 20$, and the computation overhead of the step size scaling is negligible. The number of total substitution 
operations is 
\begin{eqnarray}
    \sum_{i=0}^N m_{i}, \nonumber
\end{eqnarray}
where $N$ is total time steps, and $m_i$ is required dimension of rational Krylov subspace of each time step. Compared to 
the trapezoidal method where the number of substitution operations depends on the fixed step size, MEXP could use less 
substitution operations as long as the maximum allowed step size is much larger than the fixed step size. Our experiments 
in the following section demonstrates it is usually the case for the power grid simulation.


==> copyright.tex <==
\noindent 
Copyright (c) 2015 IEEE. Personal use of this material is permitted. However, permission to use
this material for any other purposes must be obtained from the IEEE by sending an email to
pubs-permissions@ieee.org.
\newpage 

==> drmatex.tex <==
\subsubsection{Motivation}
With the ability of large step time-marching, the input term $\mbf b$ embedded in Eq. (\ref{eqn:discrete_sol}) actually serves a double-edged sword in MEVP computation. There are usually many input currents in PDNs as well as their breakpoints, which narrow the regions for the time stepping of matrix exponential-based method due to the unaligned breakpoints. The region before the next transition $t_s$ may be shortened when there are a lot of independent input sources injected into the linear system. It leads to more chances of generating new Krylov subspace. We want to reduce the number of  Krylov subspace generations to improve the runtime performance. \footnote{%\bf 
The breakpoints also put the constraint on TR-FTS and other low order integration schemes (Backward Euler, etc.). However, the incapability of large step time-marching and theoretical limitations of low order accuracy refrain them from reaching this problem in the first place.}
\vspace{+0.1in}

\subsubsection{Treatment and Methodology} 
\label{ltsgts}
% In order to solve the frequent breakpoints problem by distributed computing, 
In matrix exponential integration framework, the flexible time stepping can choose any time spot until the next input transition spot $t_s$, as long as the 
%matrix exponential and vector 
approximation of $e^{\mbf A}\mbf v$
is accurate enough. The Krylov subspace can be reused 
when $t+h \in [t,t_s]$, only by scaling $\mbf H_m$ with $h$ 
in 
$$\mbf x(t+h) = \lVert \mbf v \rVert \mbf {V_m} e^{h \mbf H_m} \mbf e_1-\mbf P(t,h).$$
This is an important feature that even doing the adaptive time stepping, we can still use the last Krylov subspaces. Since the PDN is linear dynamical system, we can utilize the well-known superposition property of linear system and distributed computing model to tackle this challenge. 

To illustrate our distributed version of MATEX framework, we first define three terms for  breakpoints  of input sources:
\vspace{+0.08in}
\begin{itemize}
\item 
%\textbf{Definition}: 
\emph{Local Transition Spot} ($LTS$): the set of $TS$ at an input source to the PDN.
\item
%  \textbf{Definition}: 
\emph{{Global Transition Spot}} ($GTS$): the union of $LTS$ among all the input sources to the PDN. 
\item  
%\textbf{Definition}: 
\emph{{Snapshot}}:  a set $GTS \setminus LTS$ at {an input source}. 
\end{itemize}
\vspace{+0.08in}

If we simulate the PDN with respective to all the inputs,
$GTS$ are the places where generations of Krylov subspace 
cannot be avoided. 
For example, there are three input sources in a PDN (Fig. \ref{fig:rc_ckt}). 
The input waveforms are shown in Fig. \ref{fig:input}.
The first line is $GTS$, which is contributed by the union of $LTS$ in input sources \#1, \#2 and \#3. However, we can partition the task into subtasks by simulating each input source individually. Then, each subtask generates Krylov subspaces based on its own $LTS$ and keeps track of $Snapshot$ for the later usage of summation via superposition. {\color{red} Between two LTS points $t$ and $t+h$,  the \emph{Snapshot} points $t+h_1 < t+h_2 < \cdots < t+h_l  \in (t, t+h]$ can reuse the Krylov subspace generated at $t$}, which is mentioned in Sec. \ref{sec:discuss}. For each node, {the chances of generation of Krylov subspaces are reduced} and the time periods of reusing these subspaces are enlarged locally, which bring huge computational benefit when processing these subtasks in parallel. {\color{red} Besides, when subtasks are assigned, there are no communication among those computing nodes, leading to so-called ``Embarrassingly Parallel" computation model.}
 
Above, we divide the simulation task by input sources. We can, more aggressively, decompose the  task according to the ``bump'' shapes within such input pulse sources.  We group the input sources which have the same (t\_delay, t\_rise, t\_fall, t\_width) into one set. 
For example, the input source \#1 of Fig. \ref{fig:input} is divided to  \#1.1 and \#1.2 in \ref{fig:ckt_ts_decomp}. The input source \#2 in  Fig. \ref{fig:ckt_ts_decomp} is divided to  \#2.1 and \#2.2 in Fig. \ref{fig:ckt_ts_decomp}.  Therefore, there are four groups in Fig. \ref{fig:ckt_ts_decomp}, Group 1 contains $LTS\#1.1$, Group 2 contains $LTS\#2.1$, Group 3 contains $LTS \#2.2$, and Group 4 contains $LTS \#1.2$ and $\#3$. Our proposed framework MATEX is shown in Fig. \ref{fig:drmatex}. After pre-computing $GTS$ and decomposing $LTS$ based on ``bump'' shape (Fig. \ref{fig:ckt_ts_decomp}), we group them and form $LTS$ $\#1 \sim \#K$.\footnote{There are alternative decomposition strategies. It is also easy to extend the work  to deal with different input waveforms. We try to keep this part as simple as possible to emphasize our framework}  

MATEX scheduler sends out $GTS$ and $LTS$ to different MATEX slave node.
Then the simulations are  performed in parallel.
There are still no communications among nodes before the ``write back'' (in Fig. \ref{fig:drmatex}), by when all nodes complete their transient simulations.
Within each slave node, ``circuit solver'' (Alg. \ref{algo:ckt_solver}) 
computes transient response with varied time steps. 
Solutions are obtained without re-factorizing matrix during the transient computing. 
After finishing all simulations from slave nodes, they writes back the results
and informs the MATEX scheduler.
\begin{figure*}[ht]
\centering{
\includegraphics[width=0.8\textwidth]%{./figs/hierachical_ckt_sim.eps}
{./figs/hierachical_ckt_sim_new.eps}
%\vspace{-0.2in}
\centering{
\caption{DR-MATEX: the distributed MATEX framework using R-MATEX circuit solver}
}
\label{fig:drmatex}
}
\end{figure*}
%\textbf{Why does MATEX can leverage such distributed computing framework, but trditional methods cannot?}

\begin{figure}[ht] 
    \centering
    \includegraphics[width=3.0in]{./figs/rc_ckt.eps}
     \caption{Part of a PDN model with input sources from Fig. \ref{fig:input}.}
	\label{fig:rc_ckt}
\end{figure}

\begin{figure}[ht] 
%\scriptsize
    \centering
    \includegraphics[width=3.7in]%{./figs/time_spots.eps}
    {./figs/time_spots_2.eps}
      %  \vspace{-0.15in}
    \caption{
	{ 
	{Illustration of input transitions. 
	GTS: Global Transition Spots; LTS: Local Transition Spots;
	{\bf Snapshots: the crossing positions by dash lines and LTS \#$k$ without solid points.} 
	%that is the snapshots at LTS \#$k$. % which is the set of $GTS \setminus LTS$. 
	}
	}
    }
    \label{fig:input}
\end{figure}
%\vspace{-0.03in}


\begin{figure}[ht]
%\scriptsize
    \centering
    \includegraphics[width=3.65in]%{./figs/ckt_ts_decomp.eps}
    {./figs/source_large.eps}
    %   \vspace{-0.15in}
    \caption{ 
	{Grouping of ``Bump'' shape transitions for sub-task simulation.
	The matrix exponential-based method can  utilize  adaptive stepping in each LTS and reuse the Krylov subspace generated at the most recent solid point. 
	However, traditional methods (TR, BE, etc) still need to do time marching step by step, either by pairs of backward and forward substitutions and proceed with fixed time step, or re-factorize matrix and solve linear system when using adaptive stepping. 
	    (Pulse input information:
	        t\_delay: initial delay time;
	        t\_rise: rise time;
	        t\_width: width of pulse-wise; 
	        t\_fall: fall time; and
	        t\_period: period).
	}
    }
	\label{fig:ckt_ts_decomp}
\end{figure}

\begin{algorithm}
\label{algo:ckt_solver} 
{ 
\caption{DR-MATEX: the distributed NATEX framework using R-MATEX} 
\KwIn{ $LTS$ \#$k$,  $GTS$, $\mbf X_1$, $\mbf X_2$, and $\mbf P_k$, $\mbf F_k$, which contain the corresponding $\mbf b$ for node $k$; error
tolerance $E_{tol}$, and simulation time $T$.}
%\KwOut{ $\mbf V_m, \mbf H_m,  m$ }
\KwOut{Local solution $\mbf x$ along $GTS$ in node 
$k \in [1,\cdots,S]$, where $S$ is the number of nodes}
    {   
%	[$\mbf L, \mbf U$]=LU($\mbf X_1$)\\
%	Normalize the intial vector 
	$t=T_{start}$\;
	%$s=T_{start}$\;
	$\mbf x(t) = \text{Local\_Initial\_Solution}$\;
	%$\mbf x(t) = local\_DC\_analysis$; 
%	{\tcp*{ DC for input at \#$s$}} 
	%$[\mbf L,\mbf U] = \text{LU\_Decompose}( \mbf C+\gamma \mbf G)$\;
	$[\mbf L,\mbf U] = \text{LU\_Decompose}( \mbf X_1)$\;
	\While { $t \leq T_{end}$}
	{
	Compute maximum allowed step size $h$ based on $GTS$\;
	% and	$ \alpha = \frac{2h}{\gamma}$\; 
	 {
    %\tcp{\color{blue} R-MATEX mode: acurate large step marching}
	\If{$t \in $  LTS \#$k$}
	{
	\tcc{Generate the Krylov subspace for the time point of $LTS$ and compute $\mbf x$}
%	\tcp*{Reach LTS and update $\mbf V_m, \mbf H_m, \mbf v, s$}
	$[\mbf x(t+h), \mbf V_m, \mbf H_m,\mbf v] = \text{MATEX\_Arnoldi}(\mbf L,\mbf U,\mbf X_2,$ $ h, t, \mbf x(t), \epsilon, \mbf P_k(t,h), \mbf F_k(t,h))$\;
	%\label{algo2:arnoldi}
%	Update $\mbf x(t +h) $ based on Eq. (\ref{eqn:new_exact})\; 
	$a_{lts} = t$\; 
	%\tcp{put an LTS anchor for current $t$} 
	}
	\Else{
	\tcc{Compute the $\mbf x$ at $Snapshot$ by reusing the latest Krylov subspace}
%	    \For  {$s_i \in (t_i + h,t_{i+1}]$}
	    {
	    %// Take snapshots by reusing $\mbf V_m , \mbf H_m, \mbf v$ \;
	    $h_{a} = t + h - a_{lts}$\;
	    $\mbf x(t+h) = \lVert \mbf v \rVert \mbf {V_m} e^{h_{a} \mbf H_m} \mbf e_1 - \mbf P_k(t,h)$\;
	   % \label{algo2:h}
%	    Update $\mbf x(t +h) $ based on Eq. (\ref{eqn:new_exact})\; 
	%$\lVert r_m(h) \rVert  =  \lVert \mbf v \rVert \left| h_{m+1,m} e_m^T e^{h\mbf H_m} e_1 \right|$
	    }
	}
	$t= t+h$\;
	}
}    }
}
\end{algorithm}

\subsection{Complexity Analysis} 
\label{sec:complexity} 
Suppose on average we have Krylov subspace basis dimension $m$ at each time step along the time span,
one pair of backward and forward substitutions has time complexity $T_{bs}$. 
The total time complexity of serial parts is $T_{serial}$, which includes matrix factorizations, local results collection, etc.
The matrix exponential evaluation using $\mbf H_m$ is $T_{H}$ which costs time complexity $O(m^3)$, plus extra $T_e$ to form $\mbf x$, which costs $O(n m^2)$.
%$T$, $T_s$ and $T_e$ are positive proportional to the nonzero terms in operated matrices.
Given $K$ points of $GTS$, without decomposition of input transitions,
the time complexity is 
$KmT_{bs} + K (T_{H}+ T_e)  + T_{serial}$.
%$O(KmT + K (m^3+ T_e)  + T_s)$, 
After dividing the input transitions and sending to enough computing nodes, 
we have $k$ points of $LTS$ for each node based on feature extraction and grouping 
(e.g., $k=4$ for one ``bump'' shape feature).
%suppose we have enough computing nodes to parallel process all input sets, 
The total computation complexity is 
$kmT_{bs} + K (T_{H}+ T_e)  + T_{serial}$, where  $K (T_{H}+ T_e)$ contains the portion of computing $Snapshot$.
%$O( kmT + K(m^3 + T_e) + T_s)$.
%Since no commnication required between the different processors, the extra complexity form
The speedup of distributed computing over single MATEX, 
\begin{eqnarray}
%\footnotesize 
%\text{Speedup}=\frac{ O(Km^3)+ O(Ktm)+O_{s} }  {O(Km^3)+O(ktm)+O_{s}}
\text{Speedup}=\frac{ KmT_{bs} + K(T_{H}+ T_e)+ T_{serial}}  
{ kmT_{bs}+ K(T_{H}+ T_e)+T_{serial}}.
%\text{Speedup}=\frac{ KmT + K(m^3+ T_e)+ T_{s} }  { kmT+ K(m^3+T_e)+T_{s}}
\end{eqnarray}
In R-MATEX, we have very small $m$. Besides, $T_{bs}$ is larger than $T_{H}+T_e$. 
Therefore, the most dominating part is the $KmT_{bs}$.
We can always decompose input transitions, and make $k$ very small compared to $K$.
Traditional method with fixed step size has $N$ steps for the  entire simulation.
The complexity is $NT_{bs}+T_{serial}$. Then the speedup of distributed MATEX over the ones with fixed step size is,
\begin{eqnarray}
\label{eqn:tr_spd}
%\text{Speedup}=\frac{ O(Km^3)+ O(Ktm)+O_{s} }  {O(Km^3)+O(ktm)+O_{s}}
\text{Speedup}'=\frac{NT_{bs}+T_{serial} }  { kmT_{bs}+ K(T_{H}+T_e)+T_{serial}}.
\end{eqnarray}
Usually, $N$ is much larger $K$ and $km$. 
Uniform step sizes make $N$ increase due to resolution of input transitions, 
to which $K$ is not so sensitive.
As mentioned before, $k$ can be maintained in a small number.
When elongating time span of simulation,
$N$ will increase,
however, $k$ will not change due to its irrelevance to time span 
(may bring more input transition features and increase computing nodes),
and speedups tend to become larger.
Therefore, our MATEX is more robust and has promising theoretical speedups.
\vspace{+0.2in}
